Cost-Efficient LLM Serving in the Cloud: VM Selection with KV Cache Offloading

LLM inference is essential for applications like text summarization, translation, and data analysis, but the high cost of GPU instances from Cloud Service Providers (CSPs) like AWS is a major burden. This paper proposes InferSave, a cost-efficient VM selection framework for cloud based LLM inference. InferSave optimizes KV cache offloading based on Service Level Objectives (SLOs) and workload charac teristics, estimating GPU memory needs, and recommending cost-effective VM instances. Additionally, the Compute Time Calibration Function (CTCF) improves instance selection accuracy by adjusting for discrepancies between theoretical and actual GPU performance. Experiments on AWS GPU instances show that selecting lower-cost instances without KV cache offloading improves cost efficiency by up to 73.7% for online workloads, while KV cache offloading saves up to 20.19% for offline workloads.

==> 6_related.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Resource Allocation for LLM Inference}
Cloud-Based ML Serving System 
위와 같은 연구들은 클라우드 환경에서 DeepLearning 서빙을 위한 비용 효율적인 클러스터 구성\cite{Mark}을 제안했다. 하지만 이미지 처리에 중점을 맞춰서 LLM 고유의 특성을 반영하지 못한다는 한계점들이 존재한다.
\textbf{KV Cache Offloading} 연구인 Flexgen, InfiniGen~\cite{flexgen,InfiniGen}은 제약된 GPU 메모리 환경에서 CPU 및 Disk 메모리 계층 구조를 활용하여 Key-Value(KV) 캐시를 오프로딩함으로써 처리량(Throughput)을 극대화하는 것을 목표로 한다. \cb{이러한 접근은 GPU 메모리의 병목 현상을 완화하고, 자원 사용의 효율성을 높이는 데 중요한 역할을 한다.} 특히, Flexgen~\cite{flexgen}은 대규모 모델 추론에서 CPU 메모리와 NVMe 디스크를 활용해 비용 효율성을 증대시키는 방법을 탐구했으며, InfiniGen~\cite{InfiniGen}은 GPU와 CPU 간 데이터 전송을 최적화하여 처리 속도를 개선하였다.
각각 긴입력 길이로 인해 TTFT 속도 향상을 위해 KV Cache를 offloading하는 연구, 단일 query latency 향상을 위한 대표적인 연구인 Layerkv, and RAGCache~\cite{layerkv,RAGCache}는 주로 단일 GPU 노드에서 수행되었으며, 분산 추론 환경에서의 확장성과 성능 최적화는 충분히 고려하지 않았다. 게다가, 실제 클라우드 환경에서 비용과 성능 간의 Trade-off를 체계적으로 분석하거나, 다양한 워크로드와 SLO(Service Level Objective) 요구 사항을 반영한 효율성을 탐구하지 않았다. 따라서 클라우드 기반 LLM 추론에서 자원 비용 및 성능 균형을 최적화하기 위한 실질적인 클러스터 구성 전략에 대한 연구가 필요하다.

\textbf{Cloud-Based LLM Serving Systems}의 대표적인 연구인 Melage~\cite{melange}는 다양한 GPU 유형의 비용-성능 트레이드오프를 분석하고, 요청 크기(Request Size), 요청률(Request Rate), SLO와 같은 LLM 서비스 특성을 기반으로 GPU 유형을 선택하는 프레임워크를 제안하였다. 이 연구는 GPU 선택 문제를 비용 인식(Bin Packing) 문제로 모델링하여 GPU 유형 혼합을 통해 비용 효율성을 극대화하였다. 하지만, GPU 자원 최적화에만 초점을 맞추고 CPU 및 NVMe와 같은 계층적 자원 구조 활용이나, KV 캐시 오프로딩과 같은 메모리 최적화 기법을 다루지 않았다.

결과적으로, 기존 연구들은 특정 워크로드나 자원 환경에서의 최적화를 제시했지만, 분산 클러스터 환경에서의 자원 구성 최적화와 GPU, CPU, NVMe 계층을 통합적으로 고려한 자원 배치 전략에 대해서는 한계가 있다. 특히, 클라우드 환경에서 다양한 워크로드 특성과 비용-성능 간의 균형을 자동화하여 최적화하는 접근법이 부족하다는 점에서 추가적인 연구가 필요하다.
SLO-Aware Resource Allocation in LLM Inference \cite{melange},알라딘 추가


\textit{Cost Efficient Provisioning for Cloud:}
%\textit{Resource Provisioning:}
Numerous studies have explored cost-effective VM instance resource allocation for workload processing in cloud environments~\cite{spotnik,DeepSpotCloud,Proteus,clustering-analysis2023, wang2010distributed,deochake2023cloud,kokkinos2013cost,malta2019exploring,andrzejak2010decision}.
%클라우드 환경에서 워크로드 처리를 위한 cost-effective한 VM instance 자원 할당 연구들이 수행되었다~\cite{clustering-analysis2023,wang2010distributed,deochake2023cloud,kokkinos2013cost,malta2019exploring,andrzejak2010decision,wee2011debunking}.  
%G. Fragiadakis et al.~\cite{clustering-analysis2023}은 클라우드 제공업체로 부터 수집한 VM 인스턴스 가격 번들을 기반으로 VM 클러스터 가격에 대한 컴퓨팅 비용을 계산하고 이를 바탕으로 최적의 클러스터 결정 방법을 제안한다. 하지만 위 연구는 딥러닝 워크로드를 고려하지 않았으며, 컴퓨팅 비용 계산시 CPU, RAM 및 저장 공간에 대한 컴퓨팅 비용만을 계산하였다는 한계점을 갖는다.
Fragiadakis et al.~\cite{clustering-analysis2023} \co{jk: 인트로에 클러스터 챌린지를 언급할때 사용하는 건 어떨까요?} proposed an optimal cluster determination method based on calculating computational costs for VM clusters using price bundles of VM instances collected from cloud providers. 
However, this study does not consider deep learning workloads and is limited in its computation cost calculations, focusing only on CPU, RAM, and storage space.
Wang et al.~\cite{wang2010distributed} conducted a trade-off analysis of performance and cost for different instance types in a cloud environment for various workload processing scenarios. 
This study revealed that high-performance instances are not always the best choice from a pricing perspective. 
However, it did not provide criteria for selecting the optimal instance type based on specific factors.
Furthermore, Andrzejak et al.~\cite{andrzejak2010decision} proposed a method for cost-effectively meeting user service-level agreement constraints using Spot VM instances. 
To achieve this, they presented a cost-effective decision model that comprehensively considers the price, performance, and stability of Spot VM instances.


%또한 A.Andrzejak et al.~\cite{andrzejak2010decision}는 사용자의 service-level agreement constraint를 비용-효율적으로 준수하기 위한 Spot VM 인스턴스 활용 방법을 제안하였다. 이를 위해 Spot VM 인스턴스의 가격, 성능 및 안정성을 종합적으로 고려한 비용 효율적인 의사결정 모델을 제시하였다.
%\textit{Resource Provisioning in other domains:}
%Resource provisioning is applied not only in cloud environments but also in various other fields, particularly in the domain of storage system architecture, where it is employed~\cite{DBaas,HybirdStore,byun2023analytical,storage-DBMSs}.
%Resource Provisioning은 클라우드 환경 뿐만아니라 다른 분야에서도 적용되고 있으며, 특히 스토리지 시스템 아키텍처 분야에서 활발히 적용되고 있다~\cite{DBaas,HybirdStore,byun2023analytical,storage-DBMSs}. 
%Narayanan et al.~\cite{DBaas}는 클라우드 환경에서 Cost-Effective한 데이터 배치를 위한 SSD와 HDD의 효율적인 구성 전략을 제안하였다. 
%HybridStore~\cite{HybirdStore}는 HDD와 SSD의 두 미디어의 비용 범위내 구성을 최적화하고 워크로드의 성능과 수명 요구 사항을 충족시키기 위해 장기적인 리소스 프로비저닝과 워크로드의 동적 관리를 결합한 솔루션을 제안하였다.
%H.Byun el al.~\cite{byun2023analytical}는 대용량 데이터 처리를 위해 CSD(Computational Storage Device) Cluster 구성을 제안하고, Cluster의 구성 비용 및 Host 및 CSD의 성능적 특성을 고려한 비용 대 이익에 대한 트레이드 오프를 분석하여 제한된 예산으로 CSD를 사용한 컴퓨팅 노드를 효율적으로 구축하는 방법을 제안하였다.

\begin{comment}
\textit{Availability Support for DDL Cluster:}
%Cluster 환경에서 failure로 인한 Availability를 보장하는 방법은 Check-pointing, Job migration, Replication과 같은 다양한 방법이 존재한다~\cite{fault-torlerance-survey,fault-torlerance-survey2,hibernation}. 이중 Check-pointing 기법은 가장 popular하게 사용된다. 
전통적으로 HPC와 같은 대규모 클러스터 환경에서 checkpointing 최적화 연구가 이루어 졌다~\cite{PLFS,Lazy-ckp,veloc,SCR,FTI,GPU-En-multilevel}. 
%특히 연구~\cite{veloc,SCR,FTI}는 HPC와 같은 large scale한 환경에서의 PFS로의 synchronous한 checkpoint의 I/O 오버헤드를 지적하고, asynchronous한 방법의 multi-level checkpoint 기법을 제안하여 I/O 오버헤드를 효과적으로 감소시켰다.
%또한 
최근에는 Checkpoint 기법을 DDL 학습 클러스터에 적용하는 연구들이 존재한다~\cite{Gemini,opt-ckp-restart,Desh}는 Checkpoint-Restart 기술에 의존한 DDL학습에서의 가용성 문제를 해결하였다. 

Gemini~\cite{Gemini}는 학습 클러스터의 CPU 메모리에 체크포인트를 저장하여 빠른 복구를 가능하게 하는 방법을 제안하였다. 이를 위해 최적의 체크포인트 배치 전략과 체크포인트 트래픽 스케줄링 알고리즘을 도입하여 실패 복구 확률을 극대화하고 학습 처리량에 미치는 영향을 최소화하였다.  
%\textit{Resilience for Distributed Deep Learning:}
\end{comment}
%focus on system improvements to optimize checkpoint performance. These studies highlight 
%Furthermore, there are studies in checkpoint optimization techniques for deep learning applications~\cite{eval-multi-level,CheckFreq,DeepFreeze,Wood-PyMM-ckp,check-n-run, Gemini, opt-ckp-restart,Desh}.
%또한, 딥러닝 응용을 위한 checkpoint 최적화 기술도 활발히 연구되고 있다~\cite{eval-multi-level,CheckFreq,DeepFreeze,Wood-PyMM-ckp,check-n-run, Gemini, opt-ckp-restart,Desh}

%This approach involves more frequent checkpointing than traditional epoch-based methods while minimizing runtime overhead. 

%They propose a lightweight checkpointing technique that leverages node-local storage and the local storage of neighboring nodes between the compute node and the Parallel File System (PFS).  This approach aims to reduce checkpointing overhead by efficiently utilizing available storage resources. 

%fault-tolerance 보장을 위해 HPC와 같은 대규모 클러스터는 Checkpoint 기법을 사용한다
%~\cite{PLFS,Lazy-ckp,veloc,SCR,FTI,GPU-En-multilevel}. 
%In particular, studies~\cite{veloc,SCR} focus on system improvements to optimize checkpoint performance. These studies highlight the synchronous I/O overhead of checkpoints on parallel file systems (PFS) in large-scale cluster environments like HPC. They propose multi-level checkpoint techniques using asynchronous methods, effectively reducing I/O overhead.
%Note that, they have a limitation in leveraging the memory resources of neighboring nodes in a multi-tiered environment.
%Moreover, high-speed checkpoint techniques for deep learning applications have also been proposed ~\cite{CheckFreq,eval-multi-level,DeepFreeze,check-n-run,Gemini,opt-ckp-restart,Desh}.
%{check-n-run, Gemini, opt-ckp-restart, Desh}.
%CheckFreq~\cite{CheckFreq} proposes frequent and fine-grained checkpointing as a strategy to reduce recovery time in the event of deep learning job failures. This approach involves more frequent checkpointing than traditional epoch-based methods while minimizing runtime overhead. However, it focuses on local checkpointing for single-node DL jobs, not distributed DDL jobs. 

%proposes the use of fine-grained and frequent checkpointing as a strategy to reduce recovery time in the event of potential deep learning job failures. 
%This approach involves checkpointing at a higher frequency than the conventional epoch boundary.
%By implementing fine-grained and frequent checkpointing asynchronously, while still maintaining accuracy, the runtime overhead is minimized. 
%However, it is important to note that %the approach suggested in 
%CheckFreq focuses solely on local checkpointing of a single-node DL job, rather than DDL jobs. Additionally, some studies have explored the use of multi-level checkpointing~\cite{eval-multi-level, DeepFreeze} that involves multiple storage tiers. They propose a lightweight checkpointing technique that leverages node-local storage and the local storage of neighboring nodes between the compute node and the Parallel File System (PFS). By utilizing these storage resources effectively, they aimed to minimize the overhead of checkpointing utilizing. 

%특히 연구~\cite{veloc,SCR,FTI,GPU-En-multilevel}는 Checkpoint의 성능을 최적화 하기 위한 시스템 연구이다. 이들은 HPC와 같은 large scale cluster 환경에서 PFS로의 synchronous한 checkpoint의 I/O 오버헤드를 지적하고, asynchronous한 방법의 multi-level checkpoint 기법을 제안하여 I/O 오버헤드를 효과적으로 감소시켰다.

%또한, 딥러닝 응용을 위한 고속 chckpoint 기술도 활발히 연구되었다~\cite{CheckFreq,DeepFreeze,Wood-PyMM-ckp,check-n-run, Gemini, opt-ckp-restart, Desh}
%Recent research studies such as CheckFreq~\cite{CheckFreq} and DeepFreeze~\cite{DeepFreeze} have proposed advanced checkpointing methods that aim to overlap computation and I/O in an asynchronous manner. CheckFreq introduced fine-grained checkpointing, which performs checkpointing at the iteration boundaries, corresponding to the units of forward pass and backward pass for a minibatch. 
%On the other hand, DeepFreeze presented a multi-level checkpointing mechanism that leverages storage at multiple levels, including the local storage of neighboring nodes in a high-performance computing environment.
%However, CheckFreq did not consider the utilization of the distributed environment in DDL workloads, while DeepFreeze does not incorporate a strategy to resolve cost-effective cluster configuration.
%Also, there are studies that address the issue of availability in DDL training jobs instead of relying on traditional checkpointing methods~\cite{Resilience,CPR,qiao2018fault}.
\begin{comment}
\cp{-> 
체크포인팅 대신에 어떤 방식으로 availability (fault-tolerance) 문제에 대처했는지 1~2 문장으로 서술 필요!!
}
\end{comment}
%These works recognize the increasing overhead of the checkpoint-restart approach due to the decreasing mean time between failures (MTBF).
%Nicolae et al.~\cite{Resilience} propose alternative methods such as immediate mini-batch rollback, where training is halted upon failure.
%Then a representative node is duplicated to resume training, and conduct lossy forward recovery, which completes the step of processing the mini-batch by averaging the gradient excluding the failed node.

% 체크포인팅 관련 연구들 - CheckFreq, 멀티-레벨 체크포인팅 %
\begin{comment}
    
\cp{
체크포인팅 관련 연구들: CheckFreq, multi-level ckping\\
지금 연구와 point가 살짝 달라 빼는게 좋을 것 같고.. 그냥 지우기에는 아쉬워서 related work에 넣는게 어떨까 합니다. 무엇보다 reference 수가 상당합니다.
-> 단, 현재 paper.bib에 중복된 논문들도 몇 있을 것 같아보이는데, 한번 점검 필요 있음.
}
\end{comment}
%There have been several studies related to checkpointing for availability and resiliency~\cite{eisenman2022check, bdn, dey2020optimizing, CheckFreq}.
\begin{comment}
\cred{yk: Intro에서 가지고 왔음 여기에 잘 녹여보세요!}
CheckFreq~\cite{CheckFreq} proposes the use of fine-grained and frequent checkpointing as a strategy to reduce recovery time in the event of potential deep learning job failures. 
This approach involves checkpointing at a higher frequency than the conventional epoch boundary.
By implementing fine-grained and frequent checkpointing asynchronously, while still maintaining accuracy, the runtime overhead is minimized. 
However, it is important to note that %the approach suggested in 
CheckFreq focuses solely on local checkpointing of a single-node DL job, rather than DDL jobs. 
%considering the specific challenges and requirements of DDL jobs.
%Additionally, some studies have explored the use of multi-level checkpointing~\cite{eval-multi-level, DeepFreeze} that involves multiple storage tiers. 
%These studies take advantage of the storage hierarchy in High-Performance Computing (HPC) environments. 
%They propose a lightweight checkpointing technique that leverages node-local storage and the local storage of neighboring nodes between the compute node and the Parallel File System (PFS). 
%By utilizing these storage resources effectively, they aimed to minimize the overhead of checkpointing utilizing 
%Further, these studies utilize 
%checkpointing modules such as VELOC~\cite{veloc} or SCR~\cite{SCR}, which perform checkpointing to the file system. 
%However, it should be noted that they have a limitation in that they cannot leverage the memory of neighboring nodes in a multi-level manner.
%\cp{
%\\위 단락을 Related Work에 잘 녹여내는 것도 좋아보입니다!!
%}
\end{comment}

\begin{comment}
To mitigate this, CPR~\cite{CPR}은 대규모 추천 시스템 학습에서의 partial recovery 방법을 제안한다. 학습 중 node failure로 인한 restart시, failure가 발생하지 않은 노드는 체크포인트 데이터를 로드하지 않고 계속 학습을 진행함으로써, restart overhead를 개선하였다. 
%드하지 않고 계속 진행 함으로써, failure-restart 관련 오버헤드를 개선한다. 또한 CPR은 정확도 저하를 고려한 체크포인트 저장 간격을 선택하며 학습 성능을 극대 하면서 합리적인 정확도를 유지하는 방법을 제안한다.
~\cite{Resilience} propose alternative methods such as immediate mini-batch rollback, where training is halted upon failure.
Then a representative node is duplicated to resume training, and conduct lossy forward recovery, which completes the step of processing the mini-batch by averaging the gradient excluding the failed node.
These approaches aim to provide resilience in the face of failures without the need for traditional checkpointing. 
\end{comment}






%\textit{Cost Efficient Provisioning for Cloud:}
%클라우드 환경에서 cost-effective한 워크로드 처리를 위해 VM instance 자원 할당을 탐구하는 다양한 연구들이 수행되었다~\cite{clustering-analysis2023,wang2010distributed,deochake2023cloud,kokkinos2013cost,malta2019exploring,andrzejak2010decision}.  
%G. Fragiadakis et al.~\cite{clustering-analysis2023}은 클라우드 제공업체로 부터 수집한 VM 인스턴스 가격 번들을 기반으로 VM 클러스터 가격에 대한 컴퓨팅 비용을 계산하고 이를 바탕으로 최적의 클러스터 결정 방법을 제안한다. 하지만 위 연구는 딥러닝 워크로드를 고려하지 않았으며, 컴퓨팅 비용 계산시 CPU,RAM 및 저장 공간에 대한 컴퓨팅 비용만을 계산하였다는 한계점을 갖는다. 
%H Wang et al.~\cite{wang2010distributed}은 클라우드 환경에서 다양한 워크로드 처리에 대한 Instance 유형별 성능과 비용에 대한 trade-off 분석을 수행하였다. 이를 통해 고성능의 Instance가 가격 측면에서 항상 최선의 선택이 아님을 밝혔다. 하지만 어떠한 요소를 고려하여 최적의 인스턴스를 선택해야 하는지에 대한 기준 제시하지 않았다. 
%또한 A.Andrzejak et al.~\cite{andrzejak2010decision}는 사용자의 service-level agreement constraint를 비용-효율적으로 준수하기 위한 Spot VM 인스턴스 활용 방법을 제안하였다. 이를 위해 Spot VM 인스턴스의 가격, 성능 및 안정성을 종합적으로 고려한 비용 효율적인 의사결정 모델을 제시하였다.

%S Wee.~\cite{wee2011debunking}은 Spot VM의 가격 변화에 대한 워크로드의 수행 일정 조정의 효용성에 대한 분석을 수행하였다. VM instance의 가격에 대한 시계열 분석을 통해, Spot VM instance가 표준 인스턴스 대비 상당한 비용 절감을 제공하지만, Spot VM의 가격 변동에 따른 사용자의 워크로드 일정 조정은 충분한 비용절감 효과가 없음을 밝혔다. 
%\cg{section 2리뷰하고 코멘트 합치겠음.}


%\cred{yk: 아래 단락들은 motivation에서 가지고 왔음. 여기에 나열하지요? }
%다양한 연구들이 클라우드 환경에서 cost-effective한 VM instance 자원 할당 방법을 제안해왔다.
%연구 \cite{kokkinos2013cost}에서는 AWS의 EC2 인스턴스를 사용할 때 수행중인 workload와 인스턴스들의 특성을 고려하여 작업을 배치하는 연구를 하였다.
%연구 \cite{malta2019exploring}에서는 EC2 GPU 인스턴스를 활용해 딥러닝 어플리케이션을 수행시킬 때, cost-benefit을 도입해서 어떤 인스턴스가 비용의 측면에서 더 나은지를 분석하였다.
%\cg{어떤 측면에서 cost-benefit 한지 적어주면 좋을 것 같습니다. 성능? 용량? 등등..}
%연구 \cite{andrzejak2010decision}에서는 service-level agreement constraint를 만족하면서 사용자에게 발생하는 비용을 최소로 하는 문제를 다루었다.
%그들은 Spot 인스턴스의 비용, 성능, 안정성을 고려한 decision model을 제안하였다.

%하지만, 연구 \cite{kokkinos2013cost}, \cite{andrzejak2010decision}는 DDL을 워크로드로 사용하지 않았고, \cite{malta2019exploring}는 Spot 인스턴스의 사용 가능성을 고려하지 않았다.
%본 연구에서는 DDL 워크로드를 수행하기 위해 Spot VM cluster를 비용-효율적으로 구성하는 configuration을 제안한다.

\begin{comment}
CheckFreq~\cite{CheckFreq}, DeepFreeze~\cite{DeepFreeze} 등의 연구에서는 비동기식으로 computation과 I/O를 overlap한 비동기 방식의 advanced checkpoint 방법을 제안했다.
CheckFreq은 한 minibatch에 대한 forward pass와 backward pass 수행 단위인 Iteration 바운더리로 Checkpointing을 하는 fine-grained fashion의 체크포인팅을 보여주었다.
DeepFreeze는 HPC 환경에서 neighboring nodes의 local storage를 포함한 여러 level의 storage를 활용한 multi-level checkpointing 메커니즘을 제안한다.
하지만, CheckFreq에서는 분산딥러닝 워크로드의 특성을 활용하는 것에 대한 고려는 하지 않고, DeepFreeze는 메모리에 데이터를 staging하는 설계는 채택하지 않는다.
따라서 이 paper에서 우리는 Cloud Spot VM 환경에 적합하고, data parallel 분산 딥러닝의 property를 활용하여 Level1에서 peer node의 메모리에 dnn 모델의 checkpoint data를 staging하는 방식의 \tbdfixed{} 솔루션을 제안한다.
\end{comment}
%failure에 의해 딥러닝 훈련 작업이 중단이 되었을때 작업을 다시 restart할 시, recovery time을 최소화하는
%HPC와 같은 환경을 고려한 반면 와 같이 network speed가 느린 환경을 고려하지 않았기 때문이다.



\begin{comment}
\textit{I/O Acceleration in Deep Learning:} 

Research such as HVAC~\cite{Hvac}, Shade~\cite{khan2023shade}, and DIESEL~\cite{wang2020diesel} optimize the data load of DDL by utilizing caching. HVAC accelerates I/O by caching large training data from a shared PFS to Node local or Near-node local storage when conducting DNN training in an HPC environment. 
It provides a read-only cache library that internally utilizes RPC to avoid the metadata bottleneck that occurs when processing a large number of data read requests from PFS like GPFS or Lustre. However, while these works consider the read operations on the DL dataset adequately, they lack consideration for write operations like checkpointing.
\end{comment}
\begin{comment}    
\textit{Hybrid Distributed Deep Learning Methodology:} 

DDL is an engineering concept that can be implemented in various ways. 
One approach is the combination of model parallelism and data parallelism, as proposed in ZeRO-Infinity~\cite{rajbhandari2021zero}. 
In ZeRO-Infinity, the aim is to overcome the GPU memory limitations by dividing the entire model among different GPU devices, utilizing the characteristics of model parallelism. 
Additionally, all GPU devices perform forward and backward passes for all layers of the model, demonstrating the characteristics of data parallelism.
In this approach, each GPU device holds a disjointed part of the model, and these parts are communicated to peer nodes through broadcasting, enabling learning even for the parts they do not possess. 
In terms of checkpointing strategies, two options are possible: (1) a single master node reduces all the model data and writes it to a single file, or (2) each node writes only the information of their partial model to their own storage.

\end{comment}


==> 8_ack.tex <==
\section*{Acknowledgement}
{This work was supported by the Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No.2022-0-00498, Development of high-efficiency AI computing SW core technology for high-speed processing of large learning models). This work was also supported by, and used the resources of, the Oak Ridge Leadership Computing Facility, located in the National Center for Computational Sciences at ORNL, which is managed by UT Battelle, LLC for the U.S. DOE (under the contract No. DE-AC05-00OR22725).}

==> A_artifact.tex <==
\clearpage
\begin{appendices}
\section{Artifact Description}
%: Integrating Spot and On-Demand VMs for Cost-Efficient Deep Learning Clusters in the Cloud}
\label{sec:artifact}

\subsection{Abstract}
\begin{algorithm}
\caption{Resource Suitability Evaluation and Instance Selection (Price Priority)}
\label{alg:resource-evaluation-price-first}
\SetAlgoLined

\KwIn{
    \textbf{Memory Requirements:} \\
    $\text{Mem}_{\text{model}}$ — Model weight memory requirement \\
    $\text{Mem}_{\text{activation}}$ — Activation memory requirement \\
    $\text{Mem}_{\text{KVcache}}$ — Total KV Cache memory requirement \\
    $\text{Mem}_{\text{KVcache, per\_layer}}$ — KV Cache memory per layer \\
    \textbf{For each GPU instance $i$:} \\
    $\text{GPU}_{\text{memory}}^i$ — Total GPU memory \\
    $\text{GPU}_{\text{price}}^i$ — GPU price \\
    \textbf{User-defined maximum price:} $P_{\text{max}}$
}

\KwOut{GPU candidates that satisfy both price and resource conditions}

$ \text{Candidates} \gets \emptyset$ \tcp{Initialize candidate set}

$ \text{Mem}_{\text{total}} \gets \text{Mem}_{\text{model}} + \text{Mem}_{\text{activation}} + \text{Mem}_{\text{KVcache}}$ \;
$ \text{Mem}_{\text{base}} \gets \text{Mem}_{\text{model}} + \text{Mem}_{\text{activation}}$ \;

\For{each GPU instance $i$}{
    \If{$\text{GPU}_{\text{price}}^i \leq P_{\text{max}}$}{ \tcp{Apply Price Filter}
        $ \text{Mem}_{\text{avail}}^i \gets \text{GPU}_{\text{memory}}^i - \text{Mem}_{\text{base}}$ \tcp{Calculate Available Memory}
        
        \eIf{$\text{GPU}_{\text{memory}}^i \geq \text{Mem}_{\text{total}}$}{ \tcp{Offloading Not Required}
            $ C_{\text{off}}^i \gets 0$ \;
            Add $(i, C_{\text{off}}^i)$ to Candidate Set \;
        }{
            \If{$\text{GPU}_{\text{memory}}^i < \text{Mem}_{\text{model}}$ \textbf{OR} $\text{Mem}_{\text{KVcache, per\_layer}} > \text{Mem}_{\text{avail}}^i$}{ \tcp{Offloading Not Possible}
                Mark GPU $i$ as Unsuitable \tcp{Exclude from candidates}
            }
            \Else{ \tcp{Partial KV Cache Offloading Required}
                $ C_{\text{off}}^i \gets 1 - \frac{\text{Mem}_{\text{avail}}^i}{\text{Mem}_{\text{KVcache}}}$ \;
                \If{$\text{Mem}_{\text{KVcache, per\_layer}} \leq \text{Mem}_{\text{avail}}^i$}{ \tcp{Layer-Level Constraint Check}
                    Add $(i, C_{\text{off}}^i)$ to Candidate Set \;
                }
                \Else{
                    Mark GPU $i$ as Unsuitable \tcp{Exclude from candidates}
                }
            }
        }
    }
}

Sort Candidate Set by $\text{GPU}_{\text{price}}^i$ in ascending order \;
\Return Candidate Set $\text{Candidates}$ \;
\end{algorithm}



\end{appendices}
